Bilevel Optimization for Just-in-Time Robotic Kitting and Delivery via Adaptive Task Segmentation and Scheduling

Kitting refers to the task of preparing and grouping necessary parts and tools (or "kits") for assembly in a manufacturing environment. Automating this process simplifies the assembly task for human workers and improves efficiency. Existing automated kitting systems adhere to scripted instructions and predefined heuristics. However, given variability in the availability of parts and logistic delays, the inflexibility of existing systems can limit the overall efficiency of an assembly line. In this paper, we propose a bilevel optimization framework to enable a robot to perform task segmentation-based part selection, kit arrangement, and delivery scheduling to provide custom-tailored kits just in time - i.e., right when they are needed. We evaluate the proposed approach both through a human subjects study (n=18) involving the construction of a flat-pack furniture table and shop-flow simulation based on the data from the study. Our results show that the just-in-time kitting system is objectively more efficient, resilient to upstream shop flow delays, and subjectively more preferable as compared to baseline approaches of using kits defined by rigid task segmentation boundaries defined by the task graph itself or a single kit that includes all parts necessary to assemble a single unit.

==> tables.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{2}{|c|}{} & \multicolumn{4}{c|}{Mean Time to Failure} & \multicolumn{4}{|c|}{Mean Time to Failure}\\
    \cline{3-10}
    \multicolumn{2}{|c|}{} & 30 & 60 & 90 & 120 & 30 & 60 & 90 & 120\\
    \hline
    \parbox[t]{2mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{Mean Arrival Time}}}  & \multirow{3}{*}{30} & \textbf{4372.70 (129.04)} & \textbf{4105.70 (141.02)} & \textbf{4152.80 (151.47)} & \textbf{4022.70 (144.17)} & \textbf{1035.20 (128.66)} & \textbf{716.10 (70.19)} & \textbf{681.60 (79.10)} & \textbf{621.40 (130.06)}  \\
     &  & 5257.40** (174.46) & 4638.10** (164.43) & 4331.30 (172.11) & 4212.20 (111.98) & 1780.10** (216.83) & 1211.50** (273.77) & 897.70 (227.64) & 776.80 (102.62) \\
     &  & 5079.60** (173.86) & 4433.30** (142.38) & 4313.40 (164.69) & 4300.70** (226.32) & 1931.80** (288.81) & 1262.10** (143.52) & 1149.60** (240.44) & 1016.40** (229.18) \\
    \cline{2-6}
     & \multirow{3}{*}{60} & \textbf{4609.00 (124.66)} & \textbf{4251.00 (135.65)} & \textbf{4289.40 (190.34)} & \textbf{4282.80 (152.39)} & \textbf{1289.50 (128.77)} & \textbf{861.40 (157.48)} & \textbf{862.20 (239.49)} & \textbf{854.90 (170.41)} \\
     &  & 5326.20** (241.09) & 4627.70** (135.26) & 4651.20** (115.46) & 4664.60** (192.96) & 1881.50** (234.90) & 1179.00 (168.68) & 1217.70** (237.81) & 1222.50** (249.50) \\
     &  & 5762.20** (205.53) & 5370.30** (324.03) & 5301.90** (295.83) & 5283.00** (314.16) & 2536.50** (226.92) & 2251.50** (412.17) & 2134.90** (301.54) & 2107.70** (300.58) \\
    \cline{2-6}
     & \multirow{3}{*}{90} & \textbf{4851.60 (277.47)} & \textbf{4611.10 (170.93)} & \textbf{4455.00 (216.52)} & \textbf{4587.60 (191.00)} & \textbf{1402.10 (321.81)} & \textbf{1144.30 (224.20)} & \textbf{1027.30 (253.25)} & \textbf{1202.50 (246.25)} \\
     &  & 5328.50** (182.15) & 4929.50** (142.42) & 5083.40** (152.22) & 4980.40** (237.39) & 1914.10** (276.84) & 1425.50 (143.63) & 1662.80** (188.22) & 1571.10 (307.27) \\
     &  & 5981.70** (221.53) & 5959.10** (353.97) & 5897.30** (253.95) & 5976.00** (364.24) & 2728.20** (317.71) & 2723.10** (370.88) & 2707.20** (330.04) & 2744.00** (513.12) \\
    \cline{2-6}
     & \multirow{3}{*}{120} & \textbf{4839.30 (176.64)} & \textbf{4733.50 (212.87)} & \textbf{4764.10 (196.58)} & \textbf{5010.40 (294.95)} & \textbf{1396.20 (271.32)} & \textbf{1265.30 (215.11)} & \textbf{1321.50 (297.61)} & \textbf{1550.70 (329.21)} \\
     &  & 5275.50** (188.07) & 4896.00 (237.56) & 5155.00** (306.22) & 5399.40 (365.42) & 2005.80** (138.29) & 1449.10 (246.05) & 1670.90 (308.25) & 1970.50 (412.39) \\
     &  & 5994.30** (332.51) & 6043.90** (218.83) & 6462.30** (226.59) & 6510.90** (413.18) & 2905.50** (418.61) & 2859.30** (273.99) & 3255.70** (341.55) & 3279.80** (451.55) \\
    \hline
    \end{tabular}
    \caption{Total task time of \textsl{Optimized} (top, \textbf{bold}) versus \textsl{Single Task} (middle) and \textsl{Whole Assembly} (bottom). Asterisks indicate significant differences between the indicated condition and the Optimized condition; * denotes $p < .05$ while ** denotes $p < .001.$}
    \label{tab: sim_total_task_time}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Mean Time to Failure}\\
    \hline
    30 & 60 & 90 & 120\\
    \hline
    \textbf{1035.20 (128.66)} & \textbf{716.10 (70.19)} & \textbf{681.60 (79.10)} & \textbf{621.40 (130.06)} \\
     1780.10** (216.83) & 1211.50** (273.77) & 897.70 (227.64) & 776.80 (102.62) \\
     1931.80** (288.81) & 1262.10** (143.52) & 1149.60** (240.44) & 1016.40** (229.18) \\
    \hline
     \textbf{1289.50 (128.77)} & \textbf{861.40 (157.48)} & \textbf{862.20 (239.49)} & \textbf{854.90 (170.41)} \\
     1881.50** (234.90) & 1179.00 (168.68) & 1217.70** (237.81) & 1222.50** (249.50) \\
     2536.50** (226.92) & 2251.50** (412.17) & 2134.90** (301.54) & 2107.70** (300.58) \\
    \hline
     \textbf{1402.10 (321.81)} & \textbf{1144.30 (224.20)} & \textbf{1027.30 (253.25)} & \textbf{1202.50 (246.25)} \\
     1914.10** (276.84) & 1425.50 (143.63) & 1662.80** (188.22) & 1571.10 (307.27) \\
     2728.20** (317.71) & 2723.10** (370.88) & 2707.20** (330.04) & 2744.00** (513.12) \\
    \hline
     \textbf{1396.20 (271.32)} & \textbf{1265.30 (215.11)} & \textbf{1321.50 (297.61)} & \textbf{1550.70 (329.21)} \\
     2005.80** (138.29) & 1449.10 (246.05) & 1670.90 (308.25) & 1970.50 (412.39) \\
     2905.50** (418.61) & 2859.30** (273.99) & 3255.70** (341.55) & 3279.80** (451.55) \\
    \hline
    \end{tabular}
    \caption{Human idle time of \textsl{Optimized} (top, \textbf{bold}) versus \textsl{Single Task} (middle) and \textsl{Whole Assembly} (bottom). Asterisks indicate significant differences between the indicated condition and the Optimized condition; * denotes $p < .05$ while ** denotes $p < .001.$}
    \label{tab: sim_human_idle_time}
\end{table*}
